Structure Discovery in Nonparametric Regression through Compositional Kernel Search

Despite its importance, choosing the structural form of the kernel in nonparametric regression remains a black art. We define a space of kernel structures which are built compositionally by adding and multiplying a small number of base kernels. We present a method for searching over this space of structures which mirrors the scientific discovery process. The learned structures can often decompose functions into interpretable components and enable long-range extrapolation on time-series datasets. Our structure search method outperforms many widely used kernels and kernel combination methods on a variety of prediction tasks.

==> tables/kernel_descriptions.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-02-06 18:22:55.508933
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
   & \rotatebox{0}{ Description }  & \rotatebox{0}{ Parameters }  \\ \hline
SE & Squared-exponential  & lengthscale  \\
Per & Periodic  & lengthscale, period  \\
RQ & Rational Quadratic  & lengthscale, alpha  \\
Lin & Linear  & bias  \\
\end{tabular}
\end{center}
\label{tbl:kernel_descriptions}
\end{table}


==> tables/kernels.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-03-27 09:16:04.085821
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  122.5  &  $ Lin_{0} \times Per_{0} \times CS_{0} \times CS_{0} $   \\
SE1pPer1tSE2pSE3result &  203.9  &  $ \left( SE_{0} + SE_{2} + Per_{0} \times CS_{0} \times SE_{1} \times CS_{2} \times CS_{2} \right) $   \\
SE1pRQ1result &  122.2  &  $ SE_{0} $   \\
SE1pRQ2result &  124.1  &  $ \left( SE_{0} + SE_{1} \right) $   \\
SE1pSE1pRQ1result &  98.5  &  $ SE_{0} $   \\
SE1pSE2tSE3pSE4result &  183.3  &  $ \left( SE_{1} + SE_{0} \times CS_{3} \right) \times \left( SE_{3} + Lin_{0} \times Lin_{2} \times SE_{2} \right) $   \\
SE1tSE2pSE2tSE3result &  167.8  &  $ SE_{1} \times CS_{2} \times \left( SE_{0} + SE_{1} \times SE_{2} \right) $   \\
SE1tSE2result &  119.1  &  $ SE_{0} \times SE_{1} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/kernels1d_test.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-01-31 09:31:18.867674
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
-airlineresult &  543.7  &  $ SE_{0} \times \left( LN_{0} + LN_{0} \times \left( PE_{0} + RQ_{0} \right) \right) $   \\
-solarresult &  -300.6  &  $ SE_{0} \times PE_{0} \times RQ_{0} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/kernels2.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-01-21 15:40:09.878013
\begin{table*}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
bachsynthr200fold10of10result & $ 22.6 $ & $ CB_{0} \times QD_{1} \times P3_{2} \times QD_{3} $ \\
bachsynthr200fold1of10result & $ 163.1 $ & $ QD_{0} \times QD_{2} \times \left( SE_{0} + CB_{3} \right) $ \\
bachsynthr200fold2of10result & $ 17.5 $ & $ CB_{0} \times QD_{1} \times CB_{2} \times QD_{3} $ \\
bachsynthr200fold3of10result & $ 85.3 $ & $ MT_{0} \times QD_{3} \times \left( QD_{1} + LN_{2} \right) $ \\
bachsynthr200fold4of10result & $ 15.8 $ & $ QD_{0} \times QD_{1} \times P3_{2} \times QD_{3} $ \\
bachsynthr200fold5of10result & $ 19.2 $ & $ CB_{0} \times QD_{1} \times CB_{2} \times CB_{3} $ \\
bachsynthr200fold6of10result & $ 159.9 $ & $ QD_{0} \times QD_{2} \times \left( P3_{0} + QD_{3} \right) $ \\
bachsynthr200fold7of10result & $ 170.7 $ & $ CB_{0} \times P3_{2} \times P1_{3} $ \\
bachsynthr200fold8of10result & $ 15.7 $ & $ P3_{0} \times QD_{1} \times CB_{2} \times CB_{3} $ \\
bachsynthr200fold9of10result & $ 164.3 $ & $ QD_{0} \times CB_{2} \times \left( LN_{3} + QD_{7} \right) $ \\
rconcrete500fold10of10result & $ 191.1 $ & $ MT_{1} \times RQ_{3} \times \left( RQ_{0} + P3_{7} \right) $ \\
rconcrete500fold1of10result & $ 174.6 $ & $ RQ_{1} \times RQ_{3} \times \left( RQ_{0} + MT_{7} \right) $ \\
rconcrete500fold2of10result & $ 200.2 $ & $ MT_{1} \times \left( MT_{7} + MT_{0} \times RQ_{3} \right) $ \\
rconcrete500fold3of10result & $ 203.9 $ & $ P0_{1} \times RQ_{3} \times \left( MT_{0} + MT_{7} \right) $ \\
rconcrete500fold4of10result & $ 203.0 $ & $ P0_{1} \times RQ_{3} \times \left( P0_{0} + MT_{7} \right) $ \\
rconcrete500fold5of10result & $ 284.9 $ & $ RQ_{0} \times \left( MT_{3} + MT_{7} \right) $ \\
rconcrete500fold6of10result & $ 199.3 $ & $ MT_{1} \times RQ_{3} \times \left( MT_{0} + MT_{7} \right) $ \\
rconcrete500fold7of10result & $ 268.8 $ & $ \left( MT_{7} + MT_{0} \times RQ_{3} \right) $ \\
rconcrete500fold8of10result & $ 187.5 $ & $ MT_{0} \times P0_{1} \times RQ_{3} \times P0_{7} $ \\
rconcrete500fold9of10result & $ 188.1 $ & $ RQ_{1} \times RQ_{3} \times \left( MT_{0} + MT_{7} \right) $ \\
rhousingfold10of10result & $ 130.8 $ & $ P2_{5} \times P3_{12} \times \left( RQ_{4} + LN_{6} \right) $ \\
rhousingfold1of10result & $ 135.1 $ & $ RQ_{4} \times SE_{5} \times P2_{6} \times P2_{12} $ \\
rhousingfold2of10result & $ 145.3 $ & $ SE_{5} \times P2_{12} \times \left( RQ_{4} + LN_{6} \right) $ \\
rhousingfold3of10result & $ 151.7 $ & $ RQ_{4} \times P2_{5} \times CB_{8} \times P1_{12} $ \\
rhousingfold4of10result & $ 138.2 $ & $ SE_{5} \times P2_{12} \times \left( RQ_{4} + LN_{6} \right) $ \\
rhousingfold5of10result & $ 128.7 $ & $ QD_{5} \times P1_{12} \times \left( RQ_{4} + LN_{6} \right) $ \\
rhousingfold6of10result & $ 132.5 $ & $ SE_{5} \times P1_{12} \times \left( RQ_{4} + LN_{6} \right) $ \\
rhousingfold7of10result & $  nan $ & $ CB_{3} $ \\
rhousingfold8of10result & $ 125.5 $ & $ CB_{5} \times P1_{12} \times \left( RQ_{4} + LN_{6} \right) $ \\
rhousingfold9of10result & $ 120.5 $ & $ SE_{5} \times P1_{12} \times \left( RQ_{4} + LN_{6} \right) $ \\
rpumadyn512fold10of10result & $ 397.6 $ & $ P3_{1} \times P1_{2} $ \\
rpumadyn512fold1of10result & $ 390.6 $ & $ SE_{1} \times P2_{2} $ \\
rpumadyn512fold2of10result & $ 383.2 $ & $ SE_{1} \times \left( PE_{0} + SE_{2} \right) $ \\
rpumadyn512fold3of10result & $ 404.5 $ & $ P3_{1} \times P1_{2} $ \\
rpumadyn512fold4of10result & $ 387.1 $ & $ P3_{1} \times P3_{2} $ \\
rpumadyn512fold5of10result & $ 394.3 $ & $ P3_{1} \times P3_{2} $ \\
rpumadyn512fold6of10result & $ 402.2 $ & $ P3_{1} \times P1_{2} $ \\
rpumadyn512fold7of10result & $ 396.8 $ & $ P3_{1} \times P1_{2} $ \\
rpumadyn512fold8of10result & $ 397.7 $ & $ P3_{1} \times P1_{2} $ \\
rpumadyn512fold9of10result & $ 399.2 $ & $ P3_{1} \times P1_{2} $ \\
rservofold10of10result & $ 80.3 $ & $ MT_{0} \times CB_{1} \times CB_{2} $ \\
rservofold1of10result & $ 62.8 $ & $ P0_{0} \times CB_{2} \times \left( CB_{1} + P3_{3} \right) $ \\
rservofold2of10result & $ 53.7 $ & $ MT_{0} \times CB_{2} \times \left( CB_{1} + P3_{3} \right) $ \\
rservofold3of10result & $ 41.8 $ & $ MT_{0} \times CB_{2} \times \left( CB_{1} + SE_{3} \right) $ \\
rservofold4of10result & $ 59.6 $ & $ MT_{0} \times CB_{2} \times \left( CB_{1} + P1_{3} \right) $ \\
rservofold5of10result & $ 59.9 $ & $ MT_{0} \times CB_{2} \times \left( CB_{1} + P3_{3} \right) $ \\
rservofold6of10result & $ 56.9 $ & $ MT_{0} \times CB_{2} \times \left( CB_{1} + P3_{3} \right) $ \\
rservofold7of10result & $ 68.3 $ & $ MT_{0} \times QD_{1} \times CB_{2} $ \\
rservofold8of10result & $ 38.0 $ & $ MT_{0} \times CB_{2} \times \left( CB_{1} + P3_{3} \right) $ \\
rservofold9of10result & $ 75.6 $ & $ MT_{0} \times QD_{1} \times CB_{2} $ \\
\end{tabular}
\end{center}
\end{table*}


==> tables/kernels3.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-01-22 18:16:42.933246
\begin{table*}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
bachsynthr200fold10of10result & $ 24.9 $ & $ SE_{1} \times SE_{2} \times SE_{3} \times SE_{3} \times \left( SE_{7} + SE_{0} \times SE_{0} \times SE_{1} \right) $ \\
bachsynthr200fold1of10result & $ 19.0 $ & $ SE_{0} \times SE_{0} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{3} \times SE_{3} $ \\
bachsynthr200fold2of10result & $ 21.0 $ & $ SE_{0} \times SE_{0} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{3} \times SE_{3} $ \\
bachsynthr200fold3of10result & $ 206.7 $ & $ SE_{4} \times SE_{5} $ \\
bachsynthr200fold4of10result & $ 18.2 $ & $ SE_{0} \times SE_{0} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{3} \times SE_{3} $ \\
bachsynthr200fold5of10result & $ 22.4 $ & $ SE_{0} \times SE_{0} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{3} \times SE_{3} $ \\
bachsynthr200fold6of10result & $ 20.2 $ & $ SE_{2} \times \left( SE_{0} + SE_{0} \times SE_{5} \right) \times \left( SE_{4} + SE_{0} \times SE_{1} \times SE_{3} \right) $ \\
bachsynthr200fold7of10result & $ 21.0 $ & $ SE_{0} \times SE_{0} \times SE_{3} \times \left( SE_{6} + SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \right) $ \\
bachsynthr200fold8of10result & $ 17.9 $ & $ \left( SE_{7} + SE_{0} \times SE_{0} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{3} \right) $ \\
bachsynthr200fold9of10result & $ 22.2 $ & $ SE_{0} \times SE_{0} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{3} \times SE_{3} $ \\
rconcrete500fold10of10result & $ 114.3 $ & $ SE_{0} \times SE_{6} \times \left( SE_{1} + SE_{3} \times SE_{4} \right) \times \left( SE_{3} + SE_{5} + SE_{7} \right) $ \\
rconcrete500fold1of10result & $ 127.2 $ & $ SE_{1} \times \left( SE_{0} + SE_{1} + SE_{2} \times SE_{4} \right) \times \left( SE_{3} + SE_{5} + SE_{7} \right) $ \\
rconcrete500fold2of10result & $ 155.1 $ & $ \left( SE_{1} + SE_{0} \times SE_{1} \right) \times \left( SE_{3} + SE_{7} + SE_{3} \times \left( SE_{4} + SE_{5} \right) \right) $ \\
rconcrete500fold3of10result & $ 125.8 $ & $ SE_{0} \times \left( SE_{1} + SE_{6} + SE_{3} \times SE_{4} \right) \times \left( SE_{3} + SE_{5} + SE_{7} \right) $ \\
rconcrete500fold4of10result & $ 127.0 $ & $ SE_{6} \times \left( SE_{0} + SE_{3} \right) \times \left( SE_{1} + SE_{4} \right) \times \left( SE_{3} + SE_{5} + SE_{7} \right) $ \\
rconcrete500fold5of10result & $ 125.5 $ & $ SE_{0} \times \left( SE_{3} + SE_{7} + SE_{5} \times SE_{7} \right) \times \left( SE_{4} + SE_{1} \times SE_{6} \right) $ \\
rconcrete500fold6of10result & $ 134.3 $ & $ \left( SE_{0} + SE_{3} \times SE_{4} \right) \times \left( SE_{1} + SE_{6} \right) \times \left( SE_{3} + SE_{5} + SE_{7} \right) $ \\
rconcrete500fold7of10result & $ 118.1 $ & $ \left( SE_{0} + SE_{6} \right) \times \left( SE_{1} + SE_{3} \times SE_{4} \right) \times \left( SE_{3} + SE_{5} + SE_{7} \right) $ \\
rconcrete500fold8of10result & $ 106.0 $ & $ SE_{0} \times SE_{6} \times \left( SE_{1} + SE_{3} \times SE_{4} \right) \times \left( SE_{3} + SE_{5} + SE_{7} \right) $ \\
rconcrete500fold9of10result & $ 116.7 $ & $ \left( SE_{0} + SE_{6} \right) \times \left( SE_{1} + SE_{4} \right) \times \left( SE_{5} + SE_{7} + SE_{0} \times SE_{3} \right) $ \\
rhousingfold10of10result & $ 107.6 $ & $ SE_{5} \times SE_{11} \times SE_{12} \times \left( SE_{4} + SE_{6} \times SE_{9} \times SE_{11} \times SE_{12} \right) $ \\
rhousingfold1of10result & $ 102.3 $ & $ SE_{5} \times SE_{6} \times \left( SE_{7} + SE_{9} \right) \times \left( SE_{4} \times SE_{10} + SE_{11} \times SE_{12} \right) $ \\
rhousingfold2of10result & $ 105.3 $ & $ SE_{5} \times \left( SE_{2} \times SE_{4} + SE_{6} \times SE_{11} \times SE_{12} \times \left( SE_{7} + SE_{9} \right) \right) $ \\
rhousingfold3of10result & $ 111.4 $ & $ SE_{5} \times SE_{8} \times \left( SE_{4} + SE_{0} \times \left( SE_{11} + SE_{12} \right) \right) \times \left( SE_{4} + SE_{6} \right) $ \\
rhousingfold4of10result & $ 108.4 $ & $ SE_{5} \times SE_{9} \times SE_{11} \times SE_{12} \times \left( SE_{4} + SE_{6} \times \left( SE_{4} + SE_{12} \right) \right) $ \\
rhousingfold5of10result & $ 97.4 $ & $ SE_{5} \times SE_{12} \times \left( SE_{4} + SE_{6} \times SE_{11} \times SE_{12} \times \left( SE_{4} + SE_{9} \right) \right) $ \\
rhousingfold6of10result & $ 113.9 $ & $ SE_{5} \times SE_{11} \times SE_{12} \times \left( SE_{4} + SE_{6} \times SE_{9} \times \left( SE_{5} + SE_{12} \right) \right) $ \\
rhousingfold7of10result & $ 110.8 $ & $ SE_{5} \times \left( SE_{4} + SE_{6} \times SE_{9} \times SE_{12} \right) \times \left( SE_{4} + SE_{0} \times SE_{11} \right) $ \\
rhousingfold8of10result & $ 95.1 $ & $ SE_{5} \times SE_{11} \times \left( SE_{4} + SE_{6} \times SE_{12} \times SE_{12} \times \left( SE_{4} + SE_{9} \right) \right) $ \\
rhousingfold9of10result & $ 96.6 $ & $ SE_{5} \times SE_{9} \times SE_{9} \times SE_{11} \times SE_{12} \times \left( SE_{4} + SE_{6} \times SE_{12} \right) $ \\
rpumadyn512fold10of10result & $ 397.8 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rpumadyn512fold1of10result & $ 390.8 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rpumadyn512fold2of10result & $ 392.9 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rpumadyn512fold3of10result & $ 405.2 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rpumadyn512fold4of10result & $ 387.2 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rpumadyn512fold5of10result & $ 394.4 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rpumadyn512fold6of10result & $ 402.6 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rpumadyn512fold7of10result & $ 397.4 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rpumadyn512fold8of10result & $ 399.1 $ & $ SE_{1} \times \left( SE_{1} + SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \right) $ \\
rpumadyn512fold9of10result & $ 399.8 $ & $ SE_{1} \times SE_{1} \times SE_{1} \times SE_{1} \times SE_{2} \times SE_{2} \times SE_{2} \times SE_{2} $ \\
rservofold10of10result & $ 72.3 $ & $ SE_{1} \times SE_{1} \times SE_{2} \times \left( SE_{0} + SE_{0} \right) \times \left( SE_{3} + SE_{0} \times SE_{1} \right) $ \\
rservofold1of10result & $ 70.4 $ & $ SE_{1} \times SE_{2} \times \left( SE_{0} + SE_{3} \right) \times \left( SE_{3} + SE_{0} \times \left( SE_{1} + SE_{1} \right) \right) $ \\
rservofold2of10result & $ 68.8 $ & $ SE_{1} \times SE_{2} \times \left( SE_{0} + SE_{2} \right) \times \left( SE_{3} + SE_{0} \times SE_{1} \times SE_{1} \right) $ \\
rservofold3of10result & $ 58.5 $ & $ SE_{1} \times SE_{2} \times \left( SE_{0} \times SE_{1} + SE_{0} \times SE_{0} \times SE_{3} \times SE_{3} \right) $ \\
rservofold4of10result & $ 69.8 $ & $ \left( SE_{0} + SE_{0} \times SE_{2} \times \left( SE_{0} + SE_{1} \right) \times \left( SE_{3} + SE_{0} \times SE_{1} \right) \right) $ \\
rservofold5of10result & $ 65.3 $ & $ SE_{1} \times SE_{2} \times \left( SE_{0} + SE_{0} \times SE_{1} + SE_{3} \times \left( SE_{0} + SE_{0} \right) \right) $ \\
rservofold6of10result & $ 70.8 $ & $ SE_{0} \times SE_{1} \times SE_{2} \times \left( SE_{3} + SE_{0} \times SE_{3} \times \left( SE_{1} + SE_{3} \right) \right) $ \\
rservofold7of10result & $ 62.0 $ & $ SE_{1} \times SE_{1} \times SE_{2} \times \left( SE_{0} + SE_{3} \right) \times \left( SE_{2} + SE_{0} \times SE_{0} \right) $ \\
rservofold8of10result & $ 64.1 $ & $ \left( SE_{1} + SE_{1} \times SE_{1} \times SE_{2} \times \left( SE_{0} + SE_{0} + SE_{3} \right) \right) $ \\
rservofold9of10result & $ 73.5 $ & $ SE_{2} \times \left( SE_{0} + SE_{0} \times SE_{1} \times SE_{1} \right) \times \left( SE_{0} + SE_{3} \right) $ \\
\end{tabular}
\end{center}
\end{table*}


==> tables/multi_d_additive_fig.tex <==
\begin{figure*}
\centering
\begin{tabular}{ccccc|c}
\hspace{-0.2cm}\includegraphics[width=0.2\textwidth]{../figures/additive_multi_d/additive_kernel_sum_p2.pdf} & \hspace{-0.4cm} + \hspace{-0.4cm} & 
\includegraphics[width=0.2\textwidth]{../figures/additive_multi_d/additive_kernel_sum_p1.pdf} & \hspace{-0.4cm} = \hspace{-0.4cm} & 
\includegraphics[width=0.2\textwidth]{../figures/additive_multi_d/additive_kernel.pdf} &
\includegraphics[width=0.2\textwidth]{../figures/additive_multi_d/sqexp_kernel.pdf} \\
$k_1(x_1, x_1')$ & & $k_2(x_2, x_2')$ & & $k_1(x_1,x_1') + k_2(x_2,x_2')$ &$k_1(x_1,x_1')k_2(x_2,x_2')$ \\
1D kernel & & 1D kernel & & sum of kernels & product of kernels \\ 
%& & & & & \\
%(Second Order) & & & & & Additive Kernel \\
$\downarrow$ & & $\downarrow$ & & $\downarrow$ & $\downarrow$ \\
\hspace{-0.2cm}\includegraphics[width=0.2\textwidth]{../figures/additive_multi_d/additive_kernel_draw_sum_p1.pdf}& \hspace{-0.4cm} + \hspace{-0.4cm}& 
\includegraphics[width=0.2\textwidth]{../figures/additive_multi_d/additive_kernel_draw_sum_p2.pdf}& \hspace{-0.4cm} = \hspace{-0.4cm}&
\includegraphics[width=0.2\textwidth]{../figures/additive_multi_d/additive_kernel_draw_sum.pdf} &
\includegraphics[width=0.2\textwidth]{../figures/additive_multi_d/sqexp_draw.pdf} \\
$f_1(x_1)$ & & $f_2(x_2)$ & & $f_1(x_1) + f_2(x_2)$ & $f(x_1, x_2)$ \\
draw from & & draw from & & draw from & draw from\\
1D GP prior & & 1D GP prior & & additive GP prior & product GP prior\\
%Draw from product kernel GP prior & Draw from additive kernel GP prior\\
\end{tabular}
\caption{A two-dimensional additive kernel, and a two-dimesnional product kernel.  Left: a draw from an additive kernel corresponds to a sum of draws from one-dimensional kernels.  Right: functions drawn from a product kernel prior have less long-range dependency.
%In this example, both kernels are composed of one dimensional squared-exponential kernels, but this need not be the case in general.
}
\label{fig:multi_d_additivity}
\end{figure*}


==> tables/multi_d_additive_fig_v2.tex <==
\begin{figure}
\centering
\newcommand{\fha}{2.5cm}
\newcommand{\fwa}{3.4cm}
\newcommand{\addkernpic}[1]{{\includegraphics[height=\fha,width=\fwa]{figures/additive_multi_d/#1}}}
\begin{tabular}{cc}
Kernel function & Draw from \gp{} \\
\toprule
\addkernpic{additive_kernel} & \addkernpic{additive_kernel_draw_sum} \\
$SE_1 + SE_2$ & $f_1(x_1) + f_2(x_2)$ \\
%$k_1(x_1,x_1') + k_2(x_2,x_2')$ & $f_1(x_1) + f_2(x_2)$  \\
%sum of 1D SE kernels & sum of 1D functions \\
%\midrule
\addkernpic{sqexp_kernel} & \addkernpic{sqexp_draw} \\
$SE_1 \times SE_2$ &  $f(x_1, x_2)$
%$k_1(x_1,x_1')k_2(x_2,x_2')$ & $f(x_1, x_2)$ \\
%product of & draw from\\
%1D SE kernels & product GP prior
\end{tabular}
\caption{A two-dimensional additive kernel, and a two-dimensional product kernel.  Top row: a draw from an additive kernel corresponds to a sum of draws from one-dimensional kernels.  Bottom row: functions drawn from a product kernel prior do not have a corresponding product structure.
}
\label{fig:multi_d_additivity}
\end{figure}


==> tables/regression_results_ext_combined.tex <==
% --- Automatically generated by resultsToLatex2.m ---
% Exported at 28-Jan-2013 15:53:45
\begin{table*}[ht!]
\vspace{-0.1cm}
\caption{{\small
Comparison of multidimensional regression performance. Bold results are not significantly different from the best-performing method in each experiment, in a paired t-test with a $p$-value of 5\%.
}}
\label{tbl:Regression Mean Squared Error}
{\small
\begin{center}
\begin{tabularx}{\textwidth}{l | XXXXX | XXXXX}
 & \multicolumn{5}{c}{Mean Squared Error (MSE)} & \multicolumn{5}{c}{Negative Log-Likelihood} \\
 Method & bach  & concrete  & puma  &  servo & housing
& bach  & concrete  & puma  &  servo & housing
\\ \hline
Linear Regression 
& $1.031$ & $0.404$ & $0.641$ & $0.523$ & $0.289$ 
& $2.430$ & $1.403$ & $1.881$ & $1.678$ & $1.052$ \\
\acro{GAM}
& $1.259$ & $0.149$ & $0.598$ & $0.281$ & $0.161$ 
& $1.708$ & $0.467$ & $1.195$ & $0.800$ & $0.457$ \\
\acro{HKL}
& $\mathbf{0.199}$ & $0.147$ & $0.346$ & $0.199$ & $0.151$ 
& - & - & - & - & -\\
\gp{} \acro{\kSE{}-ARD}
& $\mathbf{0.045}$ & $0.157$ & $\mathbf{0.317}$ & $\mathbf{0.126}$ & $\mathbf{0.092}$
& $\mathbf{-0.131}$ & $0.398$ & $\mathbf{0.843}$ & $0.429$ & $0.207$ \\
Additive \gp{}
& $\mathbf{0.045}$ & $\mathbf{0.089}$ & $\mathbf{0.316}$ & $\mathbf{0.110}$ & $0.102$
& $\mathbf{-0.131}$ & $\mathbf{0.114}$ & $\mathbf{0.841}$ & $0.309$ & $0.194$ \\
\hline
%$\SE{}$ 
%Structure Search & & &&&&&&&&\\
%& $\mathbf{0.044}$ & $0.089$ & $\mathbf{0.315}$ & $\mathbf{0.101}$ & $\mathbf{0.092}$ 
%& $\mathbf{-0.141}$ & $\mathbf{0.054}$ & $\mathbf{0.840}$ & $0.249$ & $\mathbf{0.147}$ \\
Search - $\SE{}, \RQ{}$
& $\mathbf{0.044}$ & $\mathbf{0.087}$ & $\mathbf{0.315}$ & $\mathbf{0.102}$ & $\mathbf{0.082}$
& $\mathbf{-0.141}$ & $\mathbf{0.065}$ & $\mathbf{0.840}$ & $0.265$ & $\mathbf{0.059}$ \\
Search - All kernels%$\SE{}, \RQ{}, \Lin{}, \Per{}$
& $\mathbf{0.509}$ & $\mathbf{0.079}$ & $\mathbf{0.321}$ & $\mathbf{0.094}$ & $\mathbf{0.112}$
& $\mathbf{0.357}$ & $\mathbf{0.114}$ & $\mathbf{0.837}$ & $\mathbf{-0.427}$ & $\mathbf{0.151}$ \\
\end{tabularx}
\end{center}
}
\end{table*}
% End automatically generated LaTeX


==> tables/regression_results_ext_mse.tex <==
% --- Automatically generated by resultsToLatex2.m ---
% Exported at 25-Apr-2013 11:50:50
\begin{table}[h!]
\caption{{\small
Regression Mean Squared Error
}}
\label{tbl:Regression Mean Squared Error}
\begin{center}
\begin{tabular}{l | r r r r r}
Method & \rotatebox{0}{ bach  }  & \rotatebox{0}{ concrete  }  & \rotatebox{0}{ puma }  & \rotatebox{0}{ servo }  & \rotatebox{0}{ housing }  \\ \hline
Linear Regression & $1.031$ & $0.404$ & $0.641$ & $0.523$ & $0.289$ \\
GP GAM & $1.259$ & $0.149$ & $0.598$ & $0.281$ & $0.161$ \\
HKL & $\mathbf{0.199}$ & $0.147$ & $0.346$ & $0.199$ & $0.151$ \\
GP Squared-exp & $\mathbf{0.045}$ & $0.157$ & $\mathbf{0.317}$ & $\mathbf{0.126}$ & $\mathbf{0.092}$ \\
GP Additive & $\mathbf{0.045}$ & $\mathbf{0.089}$ & $\mathbf{0.316}$ & $\mathbf{0.110}$ & $0.102$ \\
$\SE{}$ & $\mathbf{0.044}$ & $0.089$ & $\mathbf{0.315}$ & $\mathbf{0.101}$ & $\mathbf{0.092}$ \\
$\SE{}, \RQ{}$ & $\mathbf{0.044}$ & $\mathbf{0.087}$ & $\mathbf{0.315}$ & $\mathbf{0.102}$ & $\mathbf{0.082}$ \\
$\SE{}, \RQ{}, \Lin{}, \Per{}$ & $\mathbf{0.509}$ & $\mathbf{0.079}$ & $\mathbf{0.321}$ & $\mathbf{0.094}$ & $\mathbf{0.112}$ \\
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/regression_results_ext_nll.tex <==
% --- Automatically generated by resultsToLatex2.m ---
% Exported at 25-Apr-2013 11:50:50
\begin{table}[h!]
\caption{{\small
Regression Negative Log Likelihood
}}
\label{tbl:Regression Negative Log Likelihood}
\begin{center}
\begin{tabular}{l | r r r r r}
Method & \rotatebox{0}{ bach  }  & \rotatebox{0}{ concrete  }  & \rotatebox{0}{ puma }  & \rotatebox{0}{ servo }  & \rotatebox{0}{ housing }  \\ \hline
Linear Regression & $2.430$ & $1.403$ & $1.881$ & $1.678$ & $1.052$ \\
GP GAM & $1.708$ & $0.467$ & $1.195$ & $0.800$ & $0.457$ \\
GP Squared-exp & $\mathbf{-0.131}$ & $0.398$ & $\mathbf{0.843}$ & $0.429$ & $0.207$ \\
GP Additive & $\mathbf{-0.131}$ & $\mathbf{0.114}$ & $\mathbf{0.841}$ & $0.309$ & $0.194$ \\
$\SE{}$ & $\mathbf{-0.141}$ & $\mathbf{0.054}$ & $\mathbf{0.840}$ & $0.249$ & $\mathbf{0.147}$ \\
$\SE{}, \RQ{}$ & $\mathbf{-0.141}$ & $\mathbf{0.065}$ & $\mathbf{0.840}$ & $0.265$ & $\mathbf{0.059}$ \\
$\SE{}, \RQ{}, \Lin{}, \Per{}$ & $\mathbf{0.357}$ & $\mathbf{0.114}$ & $\mathbf{0.837}$ & $\mathbf{-0.427}$ & $\mathbf{0.151}$ \\
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/regression_results_ext_onlyall_mse.tex <==
% --- Automatically generated by resultsToLatex2.m ---
% Exported at 06-May-2013 16:48:09
\begin{table}[h!]
\caption{{\small
Regression Mean Squared Error
}}
\label{tbl:Regression Mean Squared Error}
\begin{center}
\begin{tabular}{l | r r r r r}
Method & \rotatebox{0}{ bach  }  & \rotatebox{0}{ concrete  }  & \rotatebox{0}{ puma }  & \rotatebox{0}{ servo }  & \rotatebox{0}{ housing }  \\ \hline
Linear Regression & $1.031$ & $0.404$ & $0.641$ & $0.523$ & $0.289$ \\
GP GAM & $1.259$ & $0.149$ & $0.598$ & $0.281$ & $0.161$ \\
HKL & $\mathbf{0.199}$ & $0.147$ & $0.346$ & $0.199$ & $0.151$ \\
GP Squared-exp & $\mathbf{0.045}$ & $0.157$ & $\mathbf{0.317}$ & $\mathbf{0.126}$ & $\mathbf{0.092}$ \\
GP Additive & $\mathbf{0.045}$ & $\mathbf{0.089}$ & $\mathbf{0.316}$ & $\mathbf{0.110}$ & $\mathbf{0.102}$ \\
$\SE{}, \RQ{}, \Lin{}$ & $\mathbf{0.509}$ & $\mathbf{0.079}$ & $\mathbf{0.321}$ & $\mathbf{0.094}$ & $\mathbf{0.112}$ \\
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/regression_results_ext_onlyall_nll.tex <==
% --- Automatically generated by resultsToLatex2.m ---
% Exported at 06-May-2013 16:48:09
\begin{table}[h!]
\caption{{\small
Regression Negative Log Likelihood
}}
\label{tbl:Regression Negative Log Likelihood}
\begin{center}
\begin{tabular}{l | r r r r r}
Method & \rotatebox{0}{ bach  }  & \rotatebox{0}{ concrete  }  & \rotatebox{0}{ puma }  & \rotatebox{0}{ servo }  & \rotatebox{0}{ housing }  \\ \hline
Linear Regression & $2.430$ & $1.403$ & $1.881$ & $1.678$ & $1.052$ \\
GP GAM & $1.708$ & $0.467$ & $1.195$ & $0.800$ & $0.457$ \\
GP Squared-exp & $\mathbf{-0.131}$ & $0.398$ & $\mathbf{0.843}$ & $0.429$ & $\mathbf{0.207}$ \\
GP Additive & $\mathbf{-0.131}$ & $\mathbf{0.114}$ & $\mathbf{0.841}$ & $0.309$ & $\mathbf{0.194}$ \\
$\SE{}, \RQ{}, \Lin{}$ & $\mathbf{0.357}$ & $\mathbf{0.114}$ & $\mathbf{0.837}$ & $\mathbf{-0.427}$ & $\mathbf{0.151}$ \\
\end{tabular}
\end{center}
\end{table}
% End automatically generated LaTeX


==> tables/regression_results_mse.tex <==
% --- Automatically generated by resultsToLatex2.m ---
% Exported at 28-Jan-2013 15:53:45
\begin{table*}[ht!]
\caption{{\small
Regression Mean Squared Error
}}
\label{tbl:Regression Mean Squared Error}
\begin{center}
\begin{tabular}{l | r r r r r}
Method & \rotatebox{0}{ bach  }  & \rotatebox{0}{ concrete  }  & \rotatebox{0}{ puma }  & \rotatebox{0}{ servo }  & \rotatebox{0}{ housing }  \\ \hline
Linear Regression & $1.031$ & $0.404$ & $0.641$ & $0.523$ & $0.289$ \\
GP GAM & $1.259$ & $0.149$ & $0.598$ & $0.281$ & $0.161$ \\
HKL & $\mathbf{0.199}$ & $0.147$ & $0.346$ & $0.199$ & $0.151$ \\
GP Squared-exp & $\mathbf{0.045}$ & $0.157$ & $0.317$ & $0.126$ & $\mathbf{0.092}$ \\
GP Additive & $\mathbf{0.045}$ & $\mathbf{0.089}$ & $\mathbf{0.316}$ & $\mathbf{0.110}$ & $0.102$ \\
%22-Jan & $\mathbf{0.513}$ & $\mathbf{0.089}$ & $\mathbf{0.312}$ & $\mathbf{0.095}$ & $\mathbf{0.091}$ \\
\hline
Structure Search & $\mathbf{0.044}$ & $\mathbf{0.087}$ & $\mathbf{0.315}$ & $\mathbf{0.102}$ & $\mathbf{0.082}$
\end{tabular}
\end{center}
\end{table*}
% End automatically generated LaTeX


==> tables/regression_results_nll.tex <==
% --- Automatically generated by resultsToLatex2.m ---
% Exported at 28-Jan-2013 15:53:45
\begin{table*}[ht!]
\caption{{\small
Regression Negative Log Likelihood
}}
\label{tbl:Regression Negative Log Likelihood}
\begin{center}
\begin{tabular}{l | r r r r r}
Method & \rotatebox{0}{ bach  }  & \rotatebox{0}{ concrete  }  & \rotatebox{0}{ puma }  & \rotatebox{0}{ servo }  & \rotatebox{0}{ housing }  \\ \hline
Linear Regression & $2.430$ & $1.403$ & $1.881$ & $1.678$ & $1.052$ \\
GP GAM & $1.708$ & $0.467$ & $1.195$ & $0.800$ & $0.457$ \\
GP Squared-exp & $\mathbf{-0.131}$ & $0.398$ & $0.843$ & $0.429$ & $0.207$ \\
GP Additive & $\mathbf{-0.131}$ & $\mathbf{0.114}$ & $\mathbf{0.841}$ & $\mathbf{0.309}$ & $0.194$ \\
%22-Jan & $\mathbf{0.346}$ & $\mathbf{0.134}$ & $\mathbf{0.835}$ & $\mathbf{0.241}$ & $\mathbf{0.138}$ \\
\hline
Structure Search & $\mathbf{-0.141}$ & $\mathbf{0.065}$ & $\mathbf{0.840}$ & $\mathbf{0.265}$ & $\mathbf{0.059}$
\end{tabular}
\end{center}
\end{table*}
% End automatically generated LaTeX


==> tables/simple_kernels_table.tex <==
\newcommand{\fwb}{2.45cm}  % width
\newcommand{\fwh}{1.6cm}     % height
\begin{figure}[t]
\centering
\begin{tabular}{C{\fwb}C{\fwb}C{\fwb}}
%kernel & draws from GP & GP posterior \\
\rotatebox{90}{\includegraphics[width=\fwh,height=\fwb]{../figures/structure_examples/se_kernel}} &  \includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/se_kernel_draws} & \includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/se_kernel_post} \\
squared-exp & \multicolumn{2}{c}{locally smooth} \\ \midrule
\rotatebox{90}{\includegraphics[width=\fwh,height=\fwb]{../figures/structure_examples/per_kernel}} &  \includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/per_kernel_draws} & \includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/per_kernel_post} \\
periodic & \multicolumn{2}{c}{repeated structure} \\ \midrule
\includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/lin_kernel} &  \includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/lin_kernel_draws} & \includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/lin_kernel_post} \\
linear & \multicolumn{2}{c}{linear functions} \\ \midrule
\rotatebox{90}{\includegraphics[width=\fwh,height=\fwb]{../figures/structure_examples/longse_kernel}} &  \includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/longse_kernel_draws} & \includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/longse_kernel_post} \\
long-length SE & \multicolumn{2}{c}{slowly changing}
\end{tabular}
\caption{ Properties of basic kernels.  Left: base kernels. Centre:  draws from a \gp{} with that kernel.  Right: a GP posterior after conditioning on three datapoints.
\TBD{RBG: Do we need this figure?  It's pretty standard stuff, and it's largely subsumed by Figure 2.}}
\label{fig:basic_kernels}
\end{figure}


==> tables/simple_kernels_table_v2.tex <==
\newcommand{\fwb}{1.6cm}  % width
\newcommand{\fwh}{1.2cm}     % height
\begin{figure}
\centering
\begin{tabular}{m{\fwb}m{2\fwb}}
%kernel & draws from GP & GP posterior \\
\rotatebox{90}{\includegraphics[width=\fwh,height=\fwb]{../figures/structure_examples/se_kernel}} 
& $\kernel_\textrm{SE}(\inputVar, \inputVar') = \sigma^2 \exp{\left(-\frac{(\inputVar - \inputVar')^2}{2\ell^2}\right)}$ \\
\rotatebox{90}{\includegraphics[width=\fwh,height=\fwb]{../figures/structure_examples/per_kernel}} 
& $\kernel_\textrm{Per}(\inputVar, \inputVar') = \sigma^2 \exp{\left(\frac{-2}{\ell^2}\sin^2(\frac{\pi|\inputVar - \inputVar'|}{p})\right)}$ \\
\includegraphics[width=\fwb,height=\fwh]{../figures/structure_examples/lin_kernel} 
& $\kernel_\textrm{Lin}(\inputVar, \inputVar') = \sigma_b^2 + \sigma_v^2(\inputVar - \ell)(\inputVar' - \ell)$
\end{tabular}
\caption{ Definitions of base kernels.  Left: a plot of each kernel as a function of one of its inputs.}
\label{fig:basic_kernels}
\end{figure}


==> tables/synth-12-Feb-local.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-02-13 10:36:46.192884
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  -199.9  &  $ Lin_{0} \times Per_{0} $   \\
SE1pPer1tSE2pSE3result &  -11.1  &  $ \left( SE_{0} \times SE_{2} + Per_{0} \times RQ_{1} \right) $   \\
SE1pRQ2result &  -187.2  &  $ \left( SE_{0} + RQ_{1} \right) $   \\
SE1pSE1pRQ1result &  -234.1  &  $ SE_{0} \times Per_{0} $   \\
SE1pSE2tSE3pSE4result &  -67.3  &  $ \left( SE_{0} + SE_{1} \times Per_{1} \right) \times \left( SE_{2} + SE_{3} \right) $   \\
SE1tSE2pSE2tSE3result &  -94.1  &  $ RQ_{1} \times Lin_{2} \times \left( SE_{0} + SE_{1} \times SE_{2} \right) $   \\
SE1tSE2result &  -207.7  &  $ Lin_{0} \times SE_{0} \times SE_{1} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/synth-12-Feb.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-02-13 10:34:20.628443
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  -200.6  &  $ Per_{0} \times \left( Lin_{0} + SE_{0} \right) $   \\
SE1pPer1tSE2pSE3result &  -33.4  &  $ \left( SE_{0} + SE_{2} + Per_{0} \times Lin_{1} \times RQ_{1} \right) $   \\
SE1pRQ2result &  -187.2  &  $ \left( SE_{0} + RQ_{1} \right) $   \\
SE1pSE1pRQ1result &  -234.1  &  $ SE_{0} \times Per_{0} $   \\
SE1pSE2tSE3pSE4result &  -64.5  &  $ \left( SE_{0} + SE_{1} \right) \times \left( SE_{2} + Lin_{3} \times SE_{3} \right) $   \\
SE1tSE2pSE2tSE3result &  -94.2  &  $ Lin_{0} \times SE_{1} \times \left( SE_{0} + SE_{1} \times SE_{2} \right) $   \\
SE1tSE2result &  -213.4  &  $ Lin_{0} \times SE_{0} \times Per_{0} \times SE_{1} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/synth-13-Feb-SNR-1.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-02-14 22:52:59.411302
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  448.2  &  $ Lin_{0} \times \left( SE_{0} + Per_{0} \right) $   \\
SE1pPer1tSE2pSE3result &  474.8  &  $ \left( SE_{2} + Per_{0} \times Lin_{1} \right) $   \\
SE1pRQ1result &  433.6  &  $ SE_{0} \times Per_{0} $   \\
SE1pRQ2result &  442.6  &  $ Lin_{0} \times SE_{1} $   \\
SE1pSE1pRQ1result &  430.2  &  $ SE_{0} $   \\
SE1pSE2tSE3pSE4result &  471.9  &  $ Lin_{2} \times Lin_{2} \times SE_{3} \times \left( SE_{0} + SE_{1} \right) $   \\
SE1tSE2pSE2tSE3result &  462.8  &  $ Lin_{2} \times \left( SE_{0} + SE_{1} \times SE_{2} \right) $   \\
SE1tSE2result &  442.9  &  $ Lin_{0} \times SE_{1} \times Per_{3} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/synth-13-Feb-SNR-wigglier-1.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-02-14 08:30:34.412786
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  448.0  &  $ SE_{0} \times Per_{0} \times Lin_{0} $   \\
SE1pPer1tSE2pSE3result &  480.4  &  $ \left( SE_{2} + Per_{0} \times Lin_{1} \right) $   \\
SE1pRQ1result &  433.6  &  $ SE_{0} \times Per_{0} $   \\
SE1pRQ2result &  442.6  &  $ \left( SE_{0} + SE_{1} \right) $   \\
SE1pSE2tSE3pSE4result &  525.6  &  $ SE_{0} \times SE_{3} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/synth-13-Feb-wigglier.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-02-14 17:20:49.335719
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  -201.5  &  $ \left( SE_{0} + Lin_{0} \times Per_{0} \right) $   \\
SE1pPer1tSE2pSE3result &  -9.8  &  $ \left( SE_{0} + \left( Lin_{1} + RQ_{1} \right) \times \left( SE_{2} + SE_{0} \times RQ_{1} + Per_{0} \times SE_{1} \right) \right) $   \\
SE1pRQ1result &  -195.5  &  $ RQ_{0} $   \\
SE1pRQ2result &  -182.4  &  $ \left( SE_{0} + RQ_{1} \right) $   \\
SE1pSE1pRQ1result &  -186.5  &  $ SE_{0} $   \\
SE1pSE2tSE3pSE4result &  261.7  &  $ \left( SE_{0} + SE_{1} \right) \times \left( SE_{2} + SE_{3} \right) $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/synth-13-Feb.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-02-15 00:22:37.762282
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  -199.9  &  $ Lin_{0} \times Per_{0} $   \\
SE1pPer1tSE2pSE3result &  -35.1  &  $ \left( SE_{2} + SE_{0} \times Lin_{1} + Per_{0} \times SE_{1} \right) $   \\
SE1pRQ1result &  -185.9  &  $ RQ_{0} $   \\
SE1pRQ2result &  -187.2  &  $ \left( SE_{0} + RQ_{1} \right) $   \\
SE1pSE1pRQ1result &  -234.1  &  $ SE_{0} \times Per_{0} $   \\
SE1pSE2tSE3pSE4result &  -64.5  &  $ \left( SE_{0} + SE_{1} \right) \times \left( SE_{2} + Lin_{3} \times SE_{3} \right) $   \\
SE1tSE2pSE2tSE3result &  -94.2  &  $ SE_{1} \times Lin_{2} \times \left( SE_{0} + SE_{1} \times SE_{2} \right) $   \\
SE1tSE2result &  -207.7  &  $ Lin_{0} \times SE_{0} \times SE_{1} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/synth-14-Feb-SNR-tenth.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-02-14 23:01:13.986647
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  1125.8  &  $ SE_{0} $   \\
SE1pPer1tSE2pSE3result &  1124.5  &  $ SE_{1} $   \\
SE1pRQ1result &  1106.7  &  $ Lin_{0} $   \\
SE1pRQ2result &  1102.8  &  $ Lin_{0} \times Per_{1} $   \\
SE1pSE1pRQ1result &  1103.1  &  $ SE_{0} $   \\
SE1pSE2tSE3pSE4result &  1127.4  &  $ Lin_{1} \times SE_{2} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}


==> tables/synthetic_results.tex <==
\begin{table*}[ht!]
\caption{{\small
Kernels used to generate synthetic data, dimensionality $D$ of the input space, inferred kernels, and estimated noise level.
}}
\label{tbl:synthetic-less}
\begin{center}
{\small
\begin{tabular}{c c | c c c}
%
True kernel & $D$ & Inferred kernels & Estimated $\sigma_n$ (Truth = 0.1)\\% & Temp col & Temp col \\
\hline
$\SE + \RQ$                               & 1 & $\RQ$ & 0.090 \\%& 1.06 & 0.14\\
$\Lin \times \Per$                        & 1 & $\Lin \times \Per$ & 0.098 \\%& 1.01 & 0.13\\
$\SE_1 + \RQ_2$                           & 2 & $\SE_1 + \RQ_2$ & 0.094 \\%& 0.91 & 0.14\\
$\SE_1 + \SE_2 \times \Per_1 + \SE_3$     & 3 & $\SE_1 + \SE_2 \times \Per_1 + \SE_3 \times \Lin_2$ & 0.082 \\%& 0.84 & 0.09\\
$\SE_1 \times \SE_2$                      & 4 & $\SE_1 \times \SE_2 \times \Lin_1$ & 0.103 \\%& 1.02 & \dots\\
$\SE_1 \times \SE_2 + \SE_2 \times \SE_3$ & 4 & $(\SE_1 \times \SE_2 + \SE_2 \times \SE_3) \times \Lin_3$ & 0.089 \\%& \dots & \dots\\
$(\SE_1 + \SE_2) \times (\SE_3 + \SE_4)$  & 4 & $(\SE_1 + \SE_2) \times (\SE_3 + \SE_4\times\Lin_4)$ & 0.084 \\%& 0.91 & 726\\
\end{tabular}
}
\end{center}
\end{table*}


==> tables/synthetic_results_extended.tex <==
\begin{table*}[ht!]
\caption{{\small
Kernels used to generate synthetic data together, dimensionality, $D$, of the input space and the inferred kernels at different signal to noise ratios (SNR).
The two kernels marked with an asterisk * indicate when the search procedure inferred extraneous structure.
}}
\label{tbl:synthetic}
\begin{center}
{\tiny
\begin{tabular}{c c | c c c c c}
Kernel & $D$ & SNR = 100 & SNR = 10 & SNR = 1 & SNR = 0.1 & SNR = 0.01 \\
\hline
$\SE + \RQ$                               & 1 & $\RQ$
                                              & $\SE$
                                              & $\SE \times \Per$*
                                              & $\SE$
                                              & - \\
$\Lin \times \Per$                        & 1 & $\Lin \times \Per$ 
                                              & $\Lin \times \Per$
                                              & $\Lin \times \Per$
                                              & $\SE$
                                              & - \\
$\SE_1 + \RQ_2$                           & 2 & $\SE_1 + \RQ_2$
                                              & $\SE_1 + \SE_2$
                                              & $\Lin_1 + \SE_2$ 
                                              & $\Lin_1$
                                              & - \\
$\SE_1 + \SE_2 \times \Per_1 + \SE_3$     & 3 & $\SE_1 + \SE_2 \times \Per_1 + \SE_3$
                                              & $\SE_1 + \SE_2 \times \Per_1 + \SE_3$
                                              & $\SE_2 \times \Per_1 + \SE_3$
                                              & -
                                              & - \\
$\SE_1 \times \SE_2$                      & 4 & $\SE_1 \times \SE_2 \times \Lin_1$
                                              & $\SE_1 \times \SE_2$
                                              & $\Lin_1 \times \SE_2$
                                              & $\Lin_2$
                                              & - \\
$\SE_1 \times \SE_2 + \SE_2 \times \SE_3$ & 4 & $\SE_1 \times \SE_2 + \SE_2 \times \SE_3$
                                              & $\SE_1 \times \SE_2 + \SE_2 \times \SE_3$
                                              & $\SE_1 + \SE_2 \times \SE_3$
                                              & $\SE_1$
                                              & - \\
$(\SE_1 + \SE_2) \times (\SE_3 + \SE_4)$  & 4 & $(\SE_1 + \SE_2) \times (\SE_3 + \SE_4\times\Lin_4)$
                                              & $(\SE_1 + \SE_2) \times (\SE_3\times\Lin_3\times\Lin_1 + \SE_4)$*
                                              & $(\SE_1 + \SE_2) \times \SE_3 \times \SE_4$
                                              & -
                                              & - \\
\end{tabular}
}
\end{center}
\end{table*}


==> tables/test.tex <==
%% --- Automatically generated by latex.py ---
% Exported at 2013-03-12 12:05:33.212792
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | l l l}
 Dataset  & \rotatebox{0}{ NLL }  & \rotatebox{0}{ Kernel }  \\ \hline
Lin1tPer1result &  790.6  &  $ SE_{0} $   \\
SE1pPer1tSE2pSE3result &  790.8  &  $ CS_{0} $   \\
SE1pRQ1result &  767.3  &  $ SE_{0} $   \\
SE1pRQ2result &  767.8  &  $ Lin_{0} $   \\
SE1pSE1pRQ1result &  763.6  &  $ SE_{0} $   \\
SE1pSE2tSE3pSE4result &  797.4  &  $ CS_{2} $   \\
SE1tSE2pSE2tSE3result &  788.0  &  $ SE_{0} $   \\
SE1tSE2result &  788.7  &  $ Lin_{1} $   \\
\end{tabular}
\end{center}
\label{tbl:x}
\end{table}

